Inferring COPD Severity from Tidal Breathing

Objective: To develop an algorithm that can infer the severity level of a COPD patient's airflow limitation from tidal breathing data that is collected by a wearable device. Methods: Data was collected from 25 single visit adult volunteers with a confirmed or suspected diagnosis of chronic obstructive pulmonary disease (COPD). The ground truth airflow limitation severity of each subject was determined by applying the Global Initiative for Chronic Obstructive Lung Disease (GOLD) staging criteria to the subject's spirometry results. Spirometry was performed in a pulmonary function test laboratory under the supervision of trained clinical staff. Separately, the subjects' respiratory signal was measured during quiet breathing, and a classification model was built to infer the subjects' level of airflow limitation from the measured respiratory signal. The classification model was evaluated against the ground truth using leave-one-out testing. Results: Severity of airway obstruction was classified as either mild/moderate or severe/very severe with an accuracy of 96.4%. Conclusion: Tidal breathing parameters that are measured with a wearable device can be used to distinguish between different levels of airflow limitation in COPD patients.

==> broad.tex <==
\section{Broader Impacts, Outreach and Education}

\subsection{Benefits to society}

The proposed activity will enable new and emerging applications in the field of continuous health monitoring that improve clinical practice by providing timely, accurate, patient-specific information, allowing healthcare to be proactive rather than reactive. These developments could help better manage chronic diseases, conferring benefits of (i) billions of dollars per year in reduced health care costs (ii) reduced emergency room visits and hospitalization and (iii) reduced exposure of patients to hospital-acquired infections and medical errors.

\subsection{Outreach and education plan}
Beyond the usual means of dissemination like technical conference presentations, posters, papers and journal articles, we will integrate this research into our on-going effort of broadening participation and including students from underrepresented groups (in particular women and persons of color) in STEM. Some of the activities that we have adopted are outlined below. 
\\\underline{Strategic Partnerships}\\
As the only Black person on the Dartmouth Engineering School faculty, Prof. Odame (PI) works with several offices that support underrepresented groups, including the Thayer School Inclusion and Diversity Committee, the National Society of Black Engineers, the Women in Science Program and the Society of Hispanic Professional Engineers. Odame regularly advertises student research opportunities with these offices; in turn, these offices regularly invite Odame to participate in workshops and seminars to help women and minority students navigate their career paths and adopt the appropriate resilience strategies.
\\\underline{Providing Research Experiences}\\
The Analog Lab promotes students research opportunities that combine technical rigor with socially-relevant causes, like biomedical technology for improved health-care delivery. For instance, we currently have research opportunities in wearable devices for lung function monitoring, cardiac output monitoring, lung function monitoring and diet monitoring. Projects like these have successfully recruited underrepresented groups and women, who are drawn more to fields with a direct connection to human/social concerns \cite{Martin, blackUnderrep, whysofew, Turner}. For the current proposal, we will promote student projects that address audio-based health monitoring---specifically, automatic wheeze detection and cough counting devices for monitoring chronic respiratory disease.
\\\underline{Reaching Out to Freshmen}\\
Incoming freshmen from underrepresented groups provide a unique opportunity for broadening participation: while a large percentage have a stated interest in STEM, they are often discouraged by the intimidating ``weed-out'' math and science courses that are prerequisite to starting the engineering major. To counter this unwelcoming environment, Prof. Odame has for the past 4 years participated in the Dartmouth Adventures in STEM, a week-long summer program that introduces underrepresented groups to the exciting world and possibilities that STEM presents. This program includes guest lectures, lab visits and a mini-course that
features intriguing ideas related to on-going research. The program encourages students to form an intellectual community by engaging in intellectual improvisation and discussion motivated by challenging problems posed by instructors, and by their own curiosity. This way, we have helped to increase retention of underrepresented groups in STEM. Prof. Odame will keep the program fresh and exciting by updating the material with results from the current proposed work.
\\\underline{Providing Hands-on Labs}\\
Prof. Odame is a faculty advisor for the Dartmouth College E.E. Just Program, which seeks to increase the number of underrepresented minorities at Dartmouth pursuing a degree in the STEM disciplines. Through partnership with the E.E. Just program, the Analog Lab has engaged over 80 students from underrepresented groups with hands-on engineering projects, raising interest in additional offerings like research opportunities, workshops and tutoring sessions. From the current proposed work, we will develop a lab that allows students to visualize the estimated formants of a spoken word, evaluate the quality of the estimation, and relate this to the keyword recognition accuracy of a classifier. 
\\\underline{Highlighting the Achievements of Students}\\
The Analog Lab regularly looks for opportunities to highlight the achievement of students research assistants from underrepresented groups. For example, working with the Dartmouth communications office, we have produced a number of video vignettes where women and African American men have discussed their work in the Analog Lab. Such videos, shared widely via social media, send a message that individuals from traditionally-underrepresented groups are actively involved and welcome in the Analog Lab. We will continue this tradition, and produce videos that feature underrepresented groups and their contributions to this research project.
\\\underline{Sending Representatives to Relevant Conferences}\\
The Analog Lab will look for opportunities to send representatives to conferences related to underrepresented groups. For example, we have twice presented our work at the Black in AI workshop, a venue with sponsorship from AI industry leaders (Facebook, Google, NVIDIA, etc.) that fosters collaborations and promotes initiatives to increase the presence of Black people in the field of Artificial Intelligence. Research results from the current proposed work will be relevant and of interest to the Black in AI audience.

\subsection{Broader Impact}
1. The proposed activity will help broaden the participation of groups that have traditionally been underrepresented in STEM, particularly women and people of color.\\\\
2. The proposed activities suggest various creative concepts, including forming strategic partnerships with offices that support underrepresented groups, providing research experiences, reaching out to freshmen interested in STEM, providing hands-on labs, and highlighting the research achievements of students from underrepresented groups.\\\\
3. The plan for carrying out the proposed activities will build on our previous practices that have successfully engaged students from underrepresented groups in research. We will integrate results and opportunities from the current proposed work into our already-established programs. To assess success, we will keep track of how many students from underrepresented groups are directly affiliated with the Dartmouth Analog Lab each year. For instance, in 2019, the student research assistants in the Analog Lab included two Black students (PhD), three women (1 PhD, 2 undergraduates) and one Latino student (undergraduate).\\\\
4. Prof. Odame (PI) is well-qualified to conduct the proposed activities, being the only Black person on the Dartmouth College Engineering faculty, and having worked extensively with various affinity groups for more than a decade to help improve the climate of inclusivity and diversity in Engineering, and STEM in general, at Dartmouth College.\\\\
5. There are adequate resources available and broad administrative support for these activities, as they align well with Dartmouth's institution-wide commitment to diversity in STEM. Illustrative of this support is the fact that the Dartmouth undergraduate engineering student body has been at or close to gender parity for the past 4 years (for comparison, the national average is $19\%$ women in an engineering school).


\section{Work Plan}
We will execute our proposed work with the year-by-year plan as outlined in \fig{timeline} below.

\begin{figure}[h]
\includegraphics[scale=0.75]{images/timeline.pdf}
\caption{(a) Autonomous sensors that are deployed throughout a
city can continually track pollutants, providing specific
information on when and where urban pollution peaks
\cite{Citysense} (b) (i) The dietary habits}
\label{figure:timeline}
\end{figure}


\section{Results from Prior NSF Support}

\textbf{1418497} SCH: INT: A noninvasive cardiac output device for telemonitoring ($\$829,267$; Odame, PI; Sep 2014 - Aug 2017).
This research focused on the design of an electrical impedance tomography (EIT) device for performing non-invasive cardiac imaging and cardiac output monitoring at home. 
\\\underline{Intellectual Merit:} The research resulted in three technical innovations: (1) a new approach to EIT, based on Singluar Value Decomposition, that allows imaging of the thorax
while the patient is breathing normally (2) a machine learning algorithm that can accurately extract stroke volume from noisy bioimpedance data that is collected in the unconstrained home environment (3) electronic miniaturization of the EIT system that combines signal acquisition, conditioning and digitization all onto a single integrated chip. \\\underline{Broader Impacts:} By enabling non-invasive cardiac imaging and accurate cardiac output monitoring at home, the technology that this project produced is addressing a critical barrier to progress in the effective telemonitoring of patients with chronic heart failure. A listing of the relevant publications is provided in the references \cite{takhti2019power, murphy2016signal, takhti2019structured, rao2018analog, arshad2016respiratory, murphy2019noise, takhti2016high, arshad2015towards, takhti2017high, takhti201810, rao2019current, arshad2018automated}.
